Stability of Stochastic Gradient Descent on Nonsmooth Convex Losses

Uniform stability is a notion of algorithmic stability that bounds the worst case change in the model output by the algorithm when a single data point in the dataset is replaced. An influential work of Hardt et al. (2016) provides strong upper bounds on the uniform stability of the stochastic gradient descent (SGD) algorithm on sufficiently smooth convex losses. These results led to important progress in understanding of the generalization properties of SGD and several applications to differentially private convex optimization for smooth losses. Our work is the first to address uniform stability of SGD on {\em nonsmooth} convex losses. Specifically, we provide sharp upper and lower bounds for several forms of SGD and full-batch GD on arbitrary Lipschitz nonsmooth convex losses. Our lower bounds show that, in the nonsmooth case, (S)GD can be inherently less stable than in the smooth case. On the other hand, our upper bounds show that (S)GD is sufficiently stable for deriving new and useful bounds on generalization error. Most notably, we obtain the first dimension-independent generalization bounds for multi-pass SGD in the nonsmooth case. In addition, our bounds allow us to derive a new algorithm for differentially private nonsmooth stochastic convex optimization with optimal excess population risk. Our algorithm is simpler and more efficient than the best known algorithm for the nonsmooth case Feldman et al. (2020).

==> HP_LB_GD_SGD.tex <==

\begin{thm} \label{thm:LB_GD_HP}
Let $\X={\cal B}(0,1)$, ${\cal F}={\cal F}_{\X}^0(1)$, and $d \geq C\sqrt n \log n$, for $C>0$ an absolute constant. There exists an stochastic nonsmooth convex program with underlying distribution ${\cal D}$ such that, w.h.p.~on neighbor samples $\bS,\bS^{\prime}\sim{\cal D}^n$, the full-batch gradient method (Algorithm \ref{alg:batchGD}) with constant stepsize $\eta>0$ and  $T=O(d/\sqrt n)$, has uniform hypothesis stability is lower bounded by $\delta_{\A_{\sf GD}}=\min\{1,\Omega(\eta\sqrt{T})\}$.
\end{thm}

\begin{proof}
Let $\nu,K>0$ to be determined. We consider the objective
\begin{equation} \label{eqn:GD_HP_function}
f(x,z) = \frac12\Big[\frac{1}{K}\langle z,x\rangle + \max\{0,x_1-\nu,\ldots,x_d-\nu\}\Big].
\end{equation}
For normalization purposes, we need $K\geq \sqrt d$, and we will choose it large enough so that the impact of the linear term in the norm of the iterates is negligible; given this choice, we can also set $\nu<1/[nK]$.
Consider the distribution ${\cal D}$ with independent marginals, $\bz_j\sim\mbox{Rad}$. 
This means that the risk takes the form $F_{\cal D}(x)=(1/2)\max\{0,x_1-\nu,\ldots,x_d-\nu\}$, and the empirical risk is given by
$$ F_{\bS}(x)= \frac12\Big[ \frac{1}{nK}\Big\langle \sum_{i\in[n]} \bz_i,x\Big\rangle 
+\max\{0,x_1-\nu,\ldots,x_d-\nu\} \Big].$$

W.l.o.g.~we may assume $n$ is an even number. For $j\in[d]$, consider the event $E_j=\{ \sum_{i\in[n]} \bz_j^i=0\}$, and
notice $(E_j)_{j\in[d]}$ are independent events, each of which has probability 
$p_n:= \binom{n}{n/2} 2^{-n} \approx \sqrt{2/[\pi n]}$. Given an i.i.d.~sample $\bS$,
let $\bJ$ be the set of coordinates $j\in[d]$ where $E_j$ holds, and $\bB=|\bJ|$. Clearly, $\bB$
follows a distribution $\mbox{Bin}(p_n,d)$, thus by the Chernoff bound
$$\PP[ \bB < (1/2) dp_n ] \leq \exp\{-c_1dp_n\}=\frac{1}{\mbox{poly}(n)},$$
where $c_1>0$ is an absolute constant, and the last bound holds since
$d\geq C\sqrt{n}\log(n)$. 

For constructing the neighboring dataset, we sample a coordinate $\bI\sim\Unif([n])$, and let $\bz_{\bI}^{\prime}=-\bz_{\bI}$. Now we bound the number of positive coordinates of $\bz_{\bI}$ over $\bJ$. In what follows, we implicitly condition on the set $\bJ$. Notice that the random variables $\bb_j:=\1_{\{\bz_{\bI,j}=1\}}$, $j\in\bJ$, are independent. These random variables are distributed Ber$(p_j)$ with
$p_j=\EE_{\bI}[\bb_j]
=\frac1n\sum_{i\in[n]} \1_{\{\bz_{i,j}=1\}}$. Notice furthermore that $\sum_{j\in\bJ}p_j=\bJ/2$. Finally, by the Chernoff bound
$$ \PP\Big[\sum_{j\in\bJ} \bb_j < \bJ/4\Big]=\exp\{-c_1 |\bJ|\}. $$
Conditionally on the large probability event $|\bJ|\geq (1/2)dp_n$, this event has probability $1/\mbox{poly}(n).$

Let $(x^t)_{t\in[T]}$ and $(y^t)_{t\in[T]}$ be the trajectories of the algorithm over samples $\bS$ and $\bS^{\prime}$, respectively, initialized from $x^0=y^0=0$. 
In what follows, we will ignore all coordinates outside of $\bJ$; we do this for notational convenience and also because it can be done w.l.o.g.. Indeed, subgradients of the piecewise linear term from coordinates in $\bJ^c$ always remain inactive; furthermore,
we can choose $K$ so large that the contribution of the linear term is negligible in $\|x^t\|$. 
Under the events considered above, we have that
$$F_{\bS}(x)=\frac12\max\{0,x_1-\nu,\ldots,x_d-\nu\}, \qquad 
F_{\bS^{\prime}}(x)= -\frac{1}{nK}\langle\bz_i,x\rangle+\frac12\max\{0,x_1-\nu,\ldots,x_d-\nu\}.$$
It is easy to see now that, starting from $x^0=0$, the subgradient method
applied to objective $F_{\bS}$ satisfies $x^t=0$ for all $t$. On the other hand, starting from 
$y^0=0$, the subgradient method applied to $F_{\bS^{\prime}}$ satisfies $y^1=\frac{2\eta}{nK}\bz_i$; let $\nu<\frac{2\eta}{nK}$, then
starting from this point, each step will be determined by the large subgradients on the positive orthant.
$$ y^{t+1} = \proj_{\X}\Big[y^t+\frac{\eta}{nK}\bz_i-(\eta/2) e_{j_t}\Big] \quad\forall t=1,\ldots,|\bJ|.$$
In particular, $\delta_t=\|y^t-x^t\| \geq \min\{1, \Omega(\sqrt{t}\eta)\}$, for $t=1,\ldots,dp_n/4$. The conclusion for the averaged solution follows analogously as in Theorem \ref{thm:LB_GD_basic}.
\end{proof}

The following result shows a lower bound on the uniform hypothesis stability of the fixed permutation stochastic subgradient method. Unfortunately, the construction does not work beyond $T=n$, and therefore it doesn't reproduce the exact same regimes as in Thm.~\ref{thm:LB_perm_SGD_basic}.

\begin{thm} \label{thm:LB_perm_SGD_HP}
Let $\X={\cal B}(0,1)$, ${\cal F}={\cal F}_{\X}^0(1)$, and $d \geq C n^4 \log n$, for $C>0$ an absolute constant. There exists an stochastic nonsmooth convex program with underlying distribution ${\cal D}$ such that, w.h.p.~on neighbor samples $\bS,\bS^{\prime}\sim{\cal D}^n$, the fixed permutation stochastic subgradient method (Algorithm \ref{alg:perm_SGD}) with constant stepsize $\eta>0$ and $T\leq n$, has uniform hypothesis stability lower bounded by 
$$\EE_{\boldsymbol\pi}[\delta_{\A_{\sf GD}}]=\min\left\{1,\Omega\Big(\frac{\eta T^{3/2}}{n}\Big)\right\}.$$
\end{thm}

Before presenting the proof, we remind the reader of the well-known first-passage property of the simple random walk (see, e.g. \cite[Example 2.20]{Levin:2017}): If $\bW^t$ is the simple random walk that starts at $\bW^0=0$, and $\btau=\inf\{t\geq 0: \bW^t=-1\}$ is the first passage stopping time, then 
\begin{equation} \label{eqn:first_pass_RW}\PP[\btau=2t+1]=p_t:=\frac{1}{(t+1)2^{2t+1}}\binom{2t}{t}\approx\frac{1}{2\sqrt \pi t^{3/2}}.
\end{equation}
Notice also that the probability of the first passage on an even time is zero.

\begin{proof}
We consider the function family used in Thm.~\ref{thm:LB_GD_HP}, given by \eqref{eqn:GD_HP_function}. Similarly to that proof, we set $K$ sufficiently small and $\nu<1/[nK]$.
We also consider the distribution ${\cal D}=\Unif(\{-1,+1\}^d)$, sample $\bS\stackrel{i.i.d.}{\sim}{\cal D}$, and $\bS^{\prime}$ a neighbor sample, that for $\bI\sim\Unif([n])$ satisfies $\bz_{\bI}^{\prime}=-\bz_i$. Let $(x^t)_{t\in[T]}$ and $(y^t)_{t\in[T]}$ the trajectories of Algorithm \ref{alg:perm_SGD} on $\bS,\bS^{\prime}$ respectively, both initialized at $x^0=0$. 

By the symmetry of $\bI$ under permutations and the i.i.d.~property of $\bS$, we may assume w.l.o.g. that $\boldsymbol{\pi}$ is the identity. For each coordinate $j\in[d]$, we consider the simple random walk $\bW_j^t=\sum_{i\leq t}\bz_j^i$, and the first and second passage stopping times
$$ \btau_{1j}:=\inf\{t\geq 0: \bW_j^t=-1\}; \qquad\btau_{2j}:=\inf\{ t>\btau_1(\bS):\, \bW_j^t=-1\}. $$
Notice these random walks are independent, given our assumptions on $\bS$. We partition the $d$ coordinates in blocks $B_{2t+1}$, where $t\in[n/2]$, each of size $2d/n$. For each $t\in O_n$, we lower bound the probability of first passage of some coordinate $j\in B_{2t+1}$ being equal to $t$, and never making a second passage (at least until $t=n$). Before this we compute this probability for a single $j\in B_{2t+1}$: By the strong Markov property and \eqref{eqn:first_pass_RW},

\begin{eqnarray*}
\PP[\btau_{1j}=2t+1 \,\,\wedge\,\, \btau_{2j}>n]&=&
 \PP[\btau_{1j}=2t+1] \cdot\PP[\btau_{1j}>n-(2t+1)]\\
 &=& p_t \cdot
 \PP[(\exists \tau\in\{n-t+1,\ldots,n\}: \, \btau_1=\tau]\\
 &=&p_t \cdot \sum_{i=(n-t+1)/2}^{n/2} p_{2i+1}
 \,\,=\,\, \Omega(1)\frac{1}{t^{3/2}} \big(\frac{1}{\sqrt{n-t}}-\frac{1}{\sqrt n} \big).
\end{eqnarray*}
Therefore, we can lower bound this probability by $p= \Omega(1)/[t^{3/2}n^{3/2}]=\Omega(1)/n^3$.
Now we have
$$ \PP[(\exists j\in B_{2t+1})\,\,\btau_{1j}=2t+1 \,\,\wedge\,\, \btau_{2j}>n] \geq 1-(1-p)^{d/n}
= 1-\exp\Big\{-\frac{\Omega(1)d}{n^4}\Big\}. $$
Let us denote the event above $E_{2t+1}$. By our partitioning, these events are independent, thus the probability of these simultaneous events can be bounded as
$$ \PP[\cap_{t\in[n/2]} E_{2t+1}] 
=\Big(1-\exp\Big\{-\frac{\Omega(1)d}{n^4}\Big\}\Big)^n=\big( 1-\frac{\alpha}{n}\big)^n,$$
where $\alpha=n\exp\{-\Omega(1)d/n^4\}$. We let furthermore $\alpha=1/\mbox{poly}(n)$, which leads to 
$$\PP[\cap_{t\in[n/2]} E_{2t+1}]\geq
\big(1-\frac{\alpha}{n}\big)^n \geq 1-\alpha-\frac12\frac{n(n-1)}{n^2}\alpha^2= 1-\frac{1}{\mbox{poly}(n)}.$$ Finally, for the choice of $\alpha$ above, it suffices that $d=\Omega(n^4\log n)$, which holds by assumption.

We conclude the proof by showing that under this event the algorithm will have the claimed stability lower bound. The key observation is that under the event $\cap_{t\in[n/2]} E_{2t+1}$, if $\bI=i$, then all odd iterations larger than $i$ will have one coordinate $j\in B_{2t+1}$ where only one of $x_j^t,y_j^t$ will become negative, which will make its next subgradient step $\Theta(\eta)$ in a  direction that is orthogonal to past and future steps. This leads to  

\begin{eqnarray*}
\EE_{\boldsymbol{\pi}}\|x^t-y^t\| &=&\frac1n\sum_{i=1}^{n} \EE[\|x^t-y^t\|| \bI=i]
\,\,=\,\, \frac{\Omega(1)}{n}
\sum_{i=1}^{t} \min\{1,\eta\sqrt{t-i}\}
\,\,=\,\,
\min\left\{1,\Omega\Big(\frac{\eta t^{3/2}}{n}\Big)\right\}.
\end{eqnarray*}
Analogously to the proof of Thm.~\ref{thm:LB_GD_basic}, we can obtain the same conclusion for $\barx^T$.
\end{proof}

==> main_lemma.tex <==
\subsection{A Basic Lemma}\label{sec:basic_lemma}
In the following, we state a key lemma that will be central in proving our upper bounds on UAS for the three variants we consider for gradient descent-type algorithms. 

\begin{lem}\label{lem:main_lem}
Let $(x^t)_{t\in[T]}$ and $(y^t)_{t\in[T]}$ be two sequences with $x^0=y^0$ and satisfying the recursions
\begin{eqnarray*}
x^{t+1} &=& \proj_{\X}[x^t-\eta_t g^t]\\
y^{t+1} &=& \proj_{\X}[y^t-\eta_t h^t],
\end{eqnarray*}
for all $t\in[T-1]$, where the vectors $(g^t)_{t\in[T]}$ and $(h^t)_{t\in[T]}$ lie in $\B(0, L)$ and satisfy
$$ \langle g^t-h^t,x^t-y^t\rangle \geq -a_t\|x^t-y^t\|,$$
for scalars $0\leq a_t\leq 2L$. Then
$$ \|x^T-y^T\| \leq 2L\sqrt{\sum_{t=t_0}^{T-1}\eta_t^2}+2\sum_{t=t_0+1}^{T-1}\eta_s a_s.$$
where $t_0=\inf\{t: g^t\neq h^t\}.$
\end{lem}


\begin{proof}
Let $\delta_t=\|x^t-y^t\|$. By definition of $t_0$ it is clear that $\delta_1=\ldots=\delta_{t_0}=0$. For $t=t_0+1$, we have that $\delta_{t_0+1}=\|\eta_{t_0}(g^{t_0}-h^{t_0})\|\leq 2L\eta_{t_0}$.

Now, we derive a recurrence for $(\delta_t)_{t\in[T]}$:
\begin{eqnarray*}
\delta_{t+1}^2 &=& \|\proj_{\X}[x^t-\eta_t g^t]-\proj_{\X}[y^t-\eta_t h^t]\|^2
\,\,\leq\,\, \|x^t-y^t-\eta_t( g^t- h^t)\|^2 \notag\\
&=& \delta_t^2 +\eta_t^2\|g^t-h^t\|^2
-2\eta_t\langle g^t-h^t,x^t-y^t\rangle
\,\,\leq\,\, \delta_t^2+4L^4\eta_t^2+2\eta_ta_t\delta_t.
\end{eqnarray*}
Since $\delta_{t_0+1}\leq 2L\eta_{t_0}$
\begin{eqnarray}
\delta_t^2 &\leq&  \delta_{t_0+1}^2 + 4L\sum_{s=t_0+1}^{t-1}\eta_s^2+2\sum_{s=t_0+1}^{t-1}\eta_sa_s\delta_s
\notag\\
&\leq&  4L\sum_{s=t_0}^{t-1}\eta_s^2+2\sum_{s=t_0+1}^{t-1}\eta_sa_s\delta_s.
\label{eqn:rec_stab}
\end{eqnarray}
Now we prove the following bound by induction (notice this claim proves the result):
$$ \delta_t \leq 2L\sqrt{\sum_{s=t_0}^{t-1}\eta_s^2}+2\sum_{s=t_0+1}^{t-1}\eta_sa_s\delta_s \qquad(\forall t\in[T]). $$
Indeed, the claim is clearly true for $t=t_0$. For the inductive step, we assume it holds for some $t\in[T-1]$. To prove the result we consider two cases: first, when $\delta_{t+1}\leq \max_{s\in[t]}\delta_s$, we have by induction
$$ \delta_{t+1}\leq \delta_t\leq 2L\sqrt{\sum_{s=t_0}^{t-1}\eta_s^2}+2\sum_{s=t_0+1}^{t-1}\eta_sa_s
\leq 2L\sqrt{\sum_{s=t_0}^{t}\eta_s^2}+2\sum_{s=t_0+1}^{t}\eta_sa_s. $$
In the other case, $\delta_{t+1}> \max_{s\in[t]}\delta_s$, we use \eqref{eqn:rec_stab}
$$
\delta_{t+1}^2 \,\leq\,  4L\sum_{s=t_0}^{t}\eta_t^2 + 2\sum_{s=t_0+1}^t\eta_sa_s\delta_s
\,\,\leq \,\, 4L\sum_{s=t_0}^{t}\eta_t^2 + 2\delta_{t+1}\sum_{s=t_0+1}^t\eta_sa_s,
$$
which is equivalent to 
$$\Big(\delta_{t+1}-\sum_{s=t_0+1}^ta_s\eta_s\Big)^2 \,\,\leq\,\,  4L\sum_{s=t_0}^{t}\eta_t^2 +\Big(\sum_{s=t_0+1}^t\eta_s a_s\Big)^2.
$$
Now, taking square root at the inequality, we get
\begin{eqnarray*}
\delta_{t+1}-\sum_{s=t_0+1}^ta_s\eta_s
&\leq& \sqrt{4L\sum_{s=t_0}^{t}\eta_t^2 +\Big(\sum_{s=t_0+1}^t\eta_s a_s\Big)^2}\\
&\leq& 2L\sqrt{\sum_{s=t_0}^{t}\eta_s^2} +\sum_{s=t_0+1}^t\eta_s a_s.
\end{eqnarray*}
This proves the inductive step, and therefore the result.
\end{proof}


==> recursion_Lemma.tex <==
\section{The Basic Lemma}

In the following lemma, we state a key result that will be central in proving our upper bounds on UAS for the three variants of gradient-descent algorithm. 

\begin{lem}\label{lem:main_lem}
Let $(x^t)_{t\in[T]}$ and $(y^t)_{t\in[T]}$ be two sequences with $x^0=y^0$ and satisfying the recursions
\begin{eqnarray*}
x^{t+1} &=& \proj_{\X}[x^t-\eta_t g^t]\\
y^{t+1} &=& \proj_{\X}[y^t-\eta_t h^t],
\end{eqnarray*}
for all $t\in[T-1]$, where the vectors $(g^t)_{t\in[T]}$ and $(h^t)_{t\in[T]}$ lie in $\B(0, L)$ and satisfy
$$ \langle g^t-h^t,x^t-y^t\rangle \geq -a_t\delta_t,$$
for scalars $0\leq a_t\leq 2L$. Then
$$ \|x^T-y^T\| \leq 2L\sqrt{\sum_{t=t_0}^{T-1}\eta_t^2}+2\sum_{t=t_0+1}^{T-1}\eta_s a_s.$$
where $t_0=\inf\{t: g^t\neq h^t\}.$
\end{lem}


\begin{proof}
Let $\delta_t=\|x^t-y^t\|$. By definition of $t_0$ it is clear that $\delta_1=\ldots=\delta_{t_0}=0$. For $t=t_0+1$, we have that $\delta_{t_0+1}=\|\eta_{t_0}(g^{t_0}-h^{t_0})\|\leq 2L\eta_{t_0}$.

Now, we derive a recurrence for $(\delta_t)_{t\in[T]}$:
\begin{eqnarray*}
\delta_{t+1}^2 &=& \|\proj_{\X}[x^t-\eta_t g^t]-\proj_{\X}[y^t-\eta_t h^t]\|^2
\,\,\leq\,\, \|x^t-y^y-\eta_t( g^t- h^t)\|^2 \notag\\
&=& \delta_t^2 +\eta_t^2\|g^t-h^t\|^2
-2\eta_t\langle g^t-h^t,x^t-y^t\rangle
\,\,\leq\,\, \delta_t^2+4L^4\eta_t^2+2\eta_ta_t\delta_t
\end{eqnarray*}
Since $\delta_{t_0+1}\leq 2L\eta_{t_0}$
\begin{eqnarray}
\delta_t^2 &\leq&  \delta_{t_0+1}^2 + 4L\sum_{s=t_0+1}^{t-1}\eta_s^2+2\sum_{s=t_0+1}^{t-1}\eta_sa_s\delta_s
\notag\\
&\leq&  4L\sum_{s=t_0}^{t-1}\eta_s^2+2\sum_{s=t_0+1}^{t-1}\eta_sa_s\delta_s.
\label{eqn:rec_stab}
\end{eqnarray}
Now we prove the following bound by induction (notice this claim proves the result):
$$ \delta_t \leq 2L\sqrt{\sum_{s=t_0}^{t-1}\eta_s^2}+\sum_{s=t_0+1}^{t-1}\eta_sa_s\delta_s \qquad(\forall t\in[T]). $$
Indeed, the claim is clearly true for $t=t_0$. For the inductive step, we assume it holds for some $t\in[T-1]$. To prove the result we consider two cases: first, when $\delta_{t+1}\leq \max_{s\in[t]}\delta_s$, we have by induction
$$ \delta_{t+1}\leq \delta_t\leq 2L\sqrt{\sum_{s=t_0}^{t-1}\eta_s^2}+2\sum_{s=t_0+1}^{t-1}\eta_sa_s
\leq 2L\sqrt{\sum_{s=t_0}^{t}\eta_s^2}+2\sum_{s=t_0+1}^{t}\eta_sa_s. $$
In the other case, $\delta_{t+1}> \max_{s\in[t]}\delta_s$, we use \eqref{eqn:rec_stab}
$$
\delta_{t+1}^2 \,\leq\,  4L\sum_{s=t_0}^{t}\eta_t^2 + 2\sum_{s=t_0+1}^t\eta_sa_s\delta_s
\,\,\leq \,\, 4L\sum_{s=t_0}^{t}\eta_t^2 + 2\delta_{t+1}\sum_{s=t_0+1}^t\eta_sa_s,
$$
which is equivalent to 
$$\Big(\delta_{t+1}-\sum_{s=t_0+1}^ta_s\eta_s\Big)^2 \,\,\leq\,\,  4L\sum_{s=t_0}^{t}\eta_t^2 +\Big(\sum_{s=t_0+1}^t\eta_s a_s\Big)^2.
$$
Now, taking square root at the inequality, we get
\begin{eqnarray*}
\delta_{t+1}-\sum_{s=t_0+1}^ta_s\eta_s
&\leq& \sqrt{4L\sum_{s=t_0}^{t}\eta_t^2 +\Big(\sum_{s=t_0+1}^t\eta_s a_s\Big)^2}\\
&\leq& 2L\sqrt{\sum_{s=t_0}^{t}\eta_s^2} +\sum_{s=t_0+1}^t\eta_s a_s.
\end{eqnarray*}
This proves the inductive step, and therefore the result.
\end{proof}

First, as a direct corollary of the above lemma, we derive a sharp stability bound for the batch subgradient method.

\begin{thm} \label{thm:UB_GD_}
Let $\X\subseteq\B(0,R)$ and $\F=\F_{\X}^0(L)$. The full-batch gradient descent (Algorithm \ref{alg:batchGD}) has \stabname $\delta_{\A_{\sf GD}}\leq \min\left\{2R,~
4L\,\Big(\frac1n\sum_{t=1}^{T-1}\eta_t+\sqrt{\sum_{t=1}^{T-1}\eta_t^2}\Big)\right\}$.
\end{thm}

\begin{proof} 
The bound of $2R$ is obtained directly from the diameter bound on $\X$. Therefore, we focus exclusively on the second term. Let $S\simeq S^{\prime}$, $x^0=y^0$, and consider the trajectories $(x^t)_t,(y^t)_t$ associated with the batch GD method on datasets $S$ and $S^{\prime}$, respectively. We use Lemma~\ref{lem:main_lem} with $g^t=\nabla F_{S}(x^t)$ and $h^t=\nabla F_{S^{\prime}}(y^t)$. Thus,
\begin{eqnarray*}
\langle g^t-h^t,x^t-y^t \rangle
&=&\langle \nabla F_{S}(x^t)-\nabla F_{S}(y^t),x^t-y^t \rangle +\langle \nabla F_{S}(y^t)-\nabla F_{S^{\prime}}(y^t),x^t-y^t \rangle\\
&\geq& -\|F_{S}(y^t)-\nabla F_{S^{\prime}}(y^t)\| \delta_t\\
&\geq& -\frac{2L}{n}\delta_t.
\end{eqnarray*}
where in the first inequality we used the monotonicity of the subgradient, and in the second one that $S\simeq S^{\prime}$, and that $F_{S},F_{S^{\prime}}$ are $L$-Lipschitz.

We conclude by the Lemma that for all $t\in[T]$
$$ \|x^t-y^t\| \leq 2L\sqrt{ \sum_{s=1}^{t-1}\eta_s^2 } +\frac{4L}{n}\sum_{s=1}^{t-1} \eta_s. $$
We conclude the stability bound holds for the iterates, and thus for $\overline{x}^T$ by the triangle inequality.
%Since averaging can only improve stability, we conclude the result.
\end{proof}

Next, we state and prove the following upper bounds on UAS for two variants of stochastic gradient descent: sampled-with-replacement SGD and fixed-permutation SGD. Here, we give strong upper bounds that hold with high probability (and with probability 1 in case of fixed-permutation SGD). In the appendix, we derive tighter upper bounds for these two variants of SGD in the case where the number of iterations $T < $ the number of samples in the data set $n$; however, the bounds derived in this range hold only in expectation. 

We now state and prove our upper bound for sampled-with-replacement SGD. 

\begin{thm} \label{thm:UB_repl_SGD_}
Let $\X\subseteq\B(0,R)$ and $\F=\F_{\X}^0(L)$. With probability at least $1-\exp\left(-n/2\right)$, the sampling-with-replacement stochastic gradient descent (Algorithm \ref{alg:repl_SGD}) has \stabname
$$\delta_{\A_{\sf rSGD}}\leq \min\left(2R,~ 4L\left(\sqrt{\sum_{t=1}^{T-1}\eta_t^2}  +\frac{1}{n}\sum_{t=1}^{T-1}\eta_t\right)\right).$$
\end{thm}

\begin{proof} 
The bound of $2R$ trivially follows from the diameter bound on $\X$. We thus focus on the second term of the bound. Let $S\simeq S^{\prime}$, $x^0=y^0$, and consider the trajectories $(x^t)_{t\in[T]},(y^t)_{t\in[T]}$ associated with the sampled-with-replacement stochastic subgradient method on datasets $S$ and $S^{\prime}$, respectively. We use Lemma~\ref{lem:main_lem} with $g^t=\nabla f(x^t,\bz_{\bI_t})$ and $h^t=\nabla f(y^t,\bz_{\bI_t}^{\prime})$. Let us define $\br_t\triangleq \mathbf{1}_{\{\bz_{\bI_t}\neq\bz_{\bI_t}^{\prime}\}}$. Note that at every step $t$, $\br_t=1$ with probability $1-1/n$, and $\br_t=0$ otherwise. Moreover, note that $\{\br_t: ~t\in [T]\}$ is an independent sequence of Bernoulli random variables. 

Observe,
\begin{eqnarray*}
\langle g^t-h^t,x^t-y^t \rangle
&=&\langle \nabla f(x^t,\bz_{\bI_t})-\nabla f(y^t,\bz_{\bI_t}^{\prime}),x^t-y^t \rangle\\
&\geq& -2L \br_t\delta_t.
\end{eqnarray*}
Hence, by Lemma~\ref{lem:main_lem}, for any realization of the trajectories of the SGD method, we have
\begin{align}
  \forall t\in [T]:\quad  \|x^t-y^t\| &\leq 2L\sqrt{ \sum_{s=1}^{t-1}\eta_s^2 } +4L\sum_{s=1}^{t-1} \br_s\eta_s \leq \Delta_T,\label{bound:unif_t}
\end{align}
where $\Delta_T\triangleq 2L\sqrt{ \sum_{s=1}^{T-1}\eta_s^2 } +4L\sum_{s=1}^{T-1} \br_s\eta_s$. Taking expectation of (\ref{bound:unif_t}), we have
$$ \forall t\in [T]:\quad \EE\left[\|x^t-y^t\|\right] \leq \EE\left[\Delta_T\right]= 2L\sqrt{ \sum_{s=1}^{T-1}\eta_s^2 } +\frac{4L}{n}\sum_{s=1}^{T-1}\eta_s. $$
This establishes the upper bound on UAS but only in expectation. To prove the high-probability bound, we proceed as follows. Note that each $\br_s, s\in [T],$ has variance $\frac{1}{n}\left(1-\frac{1}{n}\right)<\frac{1}{n}$. Hence, by Chernoff's bound\footnote{Here, we are applying a bound for (scaled) Bernoulli rvs where the exponent is expressed in terms of the variance.}, we have
\begin{align*}
\PP\left[\sum_{s=1}^{T-1} \br_s\eta_s \geq \frac1n\sum_{s=1}^{T-1}\eta_s+\sqrt{\sum_{s=1}^{T-1}\eta_s^2}
\right] &\leq \exp\left(-\,\frac{\sum_{s=1}^{T-1}\eta_s^2}{2\cdot\frac{1}{n}\cdot\sum_{s=1}^{T-1}\eta_s^2}\right) = \exp\left(-\frac{n}{2}\right).
\end{align*}
Therefore, with probability at least $1-\exp\left(-n/2\right)$, we have
$$\Delta_T\leq 3L\sqrt{ \sum_{s=1}^{T-1}\eta_s^2 } +\frac{4L}{n}\sum_{s=1}^{T-1}\eta_s.$$
Putting this together with (\ref{bound:unif_t}), with probability at least $1-\exp\left(-n/2\right)$, we have
$$\forall t\in [T]:\quad \|x^t-y^t\| \leq 3L\sqrt{ \sum_{s=1}^{T-1}\eta_s^2 } +\frac{4L}{n}\sum_{s=1}^{T-1}\eta_s. $$
Finally, by triangle inequality, we get that with probability at least $1-\exp\left(-n/2\right)$, the same stability bound holds for the average of the iterates $\overline{x}^T$. 
\end{proof}

Finally, we show that the same stability bound holds with probability 1 for the fixed-permutation SGD. In this result, we assume that the sequence of step sizes $\left(\eta_t\right)_{t\in [T]}$ is non-increasing, which is a valid assumption for almost all known variants of SGD.

\begin{thm} \label{thm:UB_perm_SGD_}
Let $\X\subseteq\B(0,R)$ and $\F=\F_{\X}^0(L)$. Suppose the step sizes $\left(\eta_t\right)_{t\in [T]}$ form a non-increasing sequence. Then, with probability $1$ with respect to the choice of the permutation, the fixed-permutation stochastic gradient descent (Algorithm \ref{alg:perm_SGD}) has \stabname
$$\delta_{\A_{\sf GD}}\leq \min\left\{2R,~2L \left(\sqrt{\sum_{t=1}^{T-1}\eta_t^2} +\frac{2}{n} \sum_{t=1}^{T-1}\eta_t\right)\right\}.$$
\end{thm}

\begin{proof} 
Again, the bound of $2R$ is trivial. Now, we show the second term of the bound. Let $S\simeq S^{\prime}$, $x^0=y^0$, and consider the trajectories $(x^t)_{t\in[T]},(y^t)_{t\in[T]}$ associated with the fixed permutation stochastic subgradient method on datasets $S$ and $S^{\prime}$, respectively. Fix any realized permutation $\pi$ of $[n]$ for the algorithm. Since the dataset $S$ is arbitrary, we may assume without loss of generality that $\pi$ is the identity, whereas the perturbed coordinate $\bI=i$ is arbitrary. We use Lemma~\ref{lem:main_lem} with $g^t=\nabla f\left(x^t,\bz_{\left(t ~\mbox{\footnotesize mod }n\right)}\right)$ and $h^t=\nabla f\left(y^t,\bz^{\prime}_{\left(t ~\mbox{\footnotesize mod }n\right)}\right)$. It is easy to see then that we can set $a_t$ in Lemma~\ref{lem:main_lem} as $a_t=2L \cdot\mathbf{1}_{\{(t ~\mbox{\footnotesize mod }n)=i\}}$, where $\mathbf{1}_{\{\mathsf{condition}\}}$ is the indicator of $\mathsf{condition}$. Hence, by Lemma~\ref{lem:main_lem}, we have
\begin{eqnarray*}
\|x^t-y^t\| 
&\leq& 2L\sqrt{\sum_{s=1}^{t-1}\eta_s^2} +4L\sum_{r=1}^{\lfloor (t-1)/n \rfloor}\eta_{rn+i} \\
&\leq& 2L\sqrt{\sum_{s=1}^{t-1}\eta_s^2} +\frac{4L}{n} \sum_{r=1}^{t-1}\eta_s,
\end{eqnarray*}
where at the last step we used the fact that $(\eta_t)_{t\in[T]}$ is non-increasing; namely, for any $r\geq 1$
$$ \eta_{rn+i} \leq \frac1n \sum_{s=(r-1)n+i+1}^{rn+i} \eta_s. $$
Since the bound holds for all the iterates, using triangle inequality, it holds for the output $\barx^K$ averaged over the iterates from the $T/n$ epochs.
\end{proof}
